Towards Bit-Width-Independent Proofs in SMT Solvers

Many SMT solvers implement efficient SAT-based procedures for solving fixed-size bit-vector formulas. These approaches, however, cannot be used directly to reason about bit-vectors of symbolic bit-width. To address this shortcoming, we propose a translation from bit-vector formulas of non-fixed bit-width to formulas in a logic supported by SMT solvers that includes non-linear integer arithmetic, uninterpreted functions, and universal quantification. While this logic is undecidable, this approach can still solve many formulas by capitalizing on advancements in SMT solving for non-linear arithmetic and universally quantified formulas. We provide several case studies in which we have applied this approach with promising results, including the bit-width independent verification of invertibility conditions, compiler optimizations, and bit-vector rewrites.

==> table/iv_bvsge.tex <==
{\renewcommand{\arraystretch}{1.1}%
\begin{tabular}{r@{\hspace{1em}}r}
\hline
\textbf{Literal} &  \textbf{Conditional Inverse} \\
\hline
\ensuremath{\bvsge{\bvand{x}{s}}{{t}}} & \ensuremath{\bvmaxsf} \\
\ensuremath{\bvsge{\bvlshr{x}{s}}{{t}}} & \ensuremath{\bvshl{t}{s}} \\
\ensuremath{\bvsge{\bvnot{x}}{{t}}} & \ensuremath{\bvminsf} \\
\ensuremath{\bvsge{\bvadd{x}{s}}{{t}}} & \ensuremath{\bvsub{t}{s}} \\
\ensuremath{\bvsge{\bvshl{x}{s}}{{t}}} & \ensuremath{\bvlshr{\bvmaxsf}{s}} \\
\ensuremath{\bvsge{\bvor{x}{s}}{{t}}} & \ensuremath{t} \\
\ensuremath{\bvsge{\bvurem{x}{s}}{{t}}} & \ensuremath{t} \\
\ensuremath{\bvsge{\bvurem{s}{x}}{{t}}} & \ensuremath{\bvsub{(\bvor{s}{\bvminsf})}{(\bvand{t}{\bvmaxsf})}} \\
\ensuremath{\bvsge{\bvashr{s}{x}}{{t}}} & \ensuremath{\bvand{s}{\bvminsf}} \\
\ensuremath{\bvsge{\bvashr{x}{s}}{{t}}} & \ensuremath{\bvmaxsf} \\
\ensuremath{\bvsge{\bvneg{x}}{{t}}} & \ensuremath{\bvneg{t}} \\
\hline
\end{tabular}}


==> table/iv_bvsgt.tex <==
{\renewcommand{\arraystretch}{1.1}%
\begin{tabular}{r@{\hspace{1em}}r}
\hline
\textbf{Literal} &  \textbf{Conditional Inverse} \\
\hline
\ensuremath{\bvsgt{\bvshl{x}{s}}{{t}}} & \ensuremath{\bvlshr{\bvmaxsf}{s}} \\
\ensuremath{\bvsgt{\bvashr{x}{s}}{{t}}} & \ensuremath{\bvmaxsf} \\
\ensuremath{\bvsgt{\bvnot{x}}{{t}}} & \ensuremath{\bvminsf} \\
\ensuremath{\bvsgt{\bvand{x}{s}}{{t}}} & \ensuremath{\bvmaxsf} \\
\ensuremath{\bvsgt{\bvor{x}{s}}{{t}}} & \ensuremath{\bvmaxsf} \\
\ensuremath{\bvsgt{\bvashr{s}{x}}{{t}}} & \ensuremath{\bvand{s}{\bvminsf}} \\
\ensuremath{\bvsgt{\bvlshr{x}{s}}{{t}}} & \ensuremath{\bvshl{\bvmaxsf}{s}} \\
\ensuremath{\bvsgt{\bvadd{x}{s}}{{t}}} & \ensuremath{\bvsub{\bvmaxsf}{s}} \\
\ensuremath{\bvsgt{\bvurem{s}{x}}{{t}}} & \ensuremath{\bvsub{(\bvor{s}{\bvminsf})}{(\bvand{\bvmaxsf}{\bvsub{t}{\bvmaxsf}})}} \\
\ensuremath{\bvsgt{\bvurem{x}{s}}{{t}}} & \ensuremath{\bvneg{\bvnot{t}}} \\
\ensuremath{\bvsgt{\bvneg{x}}{{t}}} & \ensuremath{\bvnot{t}} \\
\hline
\end{tabular}}


==> table/iv_bvsle.tex <==
{\renewcommand{\arraystretch}{1.1}%
\begin{tabular}{r@{\hspace{1em}}r}
\hline
\textbf{Literal} &  \textbf{Conditional Inverse} \\
\hline
\ensuremath{\bvsle{\bvashr{s}{x}}{{t}}} & \ensuremath{\bvnot{(\bvor{s}{\bvmaxsf})}} \\
\ensuremath{\bvsle{\bvashr{x}{s}}{{t}}} & \ensuremath{\bvminsf} \\
\ensuremath{\bvsle{\bvneg{x}}{{t}}} & \ensuremath{\bvminsf} \\
\ensuremath{\bvsle{\bvurem{s}{x}}{{t}}} & \ensuremath{\bvsub{s}{t}} \\
\ensuremath{\bvsle{\bvurem{x}{s}}{{t}}} & \ensuremath{\bvand{t}{\bvminsf}} \\
\ensuremath{\bvsle{\bvudiv{x}{s}}{{t}}} & \ensuremath{t} \\
\ensuremath{\bvsle{\bvnot{x}}{{t}}} & \ensuremath{\bvmaxsf} \\
\ensuremath{\bvsle{\bvor{x}{s}}{{t}}} & \ensuremath{\bvminsf} \\
\ensuremath{\bvsle{\bvand{x}{s}}{{t}}} & \ensuremath{t} \\
\ensuremath{\bvsle{\bvadd{x}{s}}{{t}}} & \ensuremath{\bvsub{t}{s}} \\
\ensuremath{\bvsle{\bvlshr{s}{x}}{{t}}} & \ensuremath{\bvnot{(\bvor{s}{\bvmaxsf})}} \\
\ensuremath{\bvsle{\bvlshr{x}{s}}{{t}}} & \ensuremath{t} \\
\ensuremath{\bvsle{\bvshl{x}{s}}{{t}}} & \ensuremath{\bvlshr{t}{s}} \\
\hline
\end{tabular}}


==> table/iv_bvslt.tex <==
{\renewcommand{\arraystretch}{1.1}%
\begin{tabular}{r@{\hspace{1em}}r}
\hline
\textbf{Literal} &  \textbf{Conditional Inverse} \\
\hline
\ensuremath{\bvslt{\bvudiv{x}{s}}{{t}}} & \ensuremath{\bvnot{\bvneg{t}}} \\
\ensuremath{\bvslt{\bvnot{x}}{{t}}} & \ensuremath{\bvmaxsf} \\
\ensuremath{\bvslt{\bvadd{x}{s}}{{t}}} & \ensuremath{\bvsub{\bvminsf}{s}} \\
\ensuremath{\bvslt{\bvashr{s}{x}}{{t}}} & \ensuremath{\bvnot{(\bvor{s}{\bvmaxsf})}} \\
\ensuremath{\bvslt{\bvashr{x}{s}}{{t}}} & \ensuremath{\bvminsf} \\
\ensuremath{\bvslt{\bvlshr{x}{s}}{{t}}} & \ensuremath{\bvshl{\bvminsf}{s}} \\
\ensuremath{\bvslt{\bvlshr{s}{x}}{{t}}} & \ensuremath{\bvnot{(\bvor{s}{\bvmaxsf})}} \\
\ensuremath{\bvslt{\bvurem{x}{s}}{{t}}} &  \\
\ensuremath{\bvslt{\bvurem{s}{x}}{{t}}} & \ensuremath{t} \\
\ensuremath{\bvslt{\bvshl{x}{s}}{{t}}} & \ensuremath{\bvlshr{\bvminsf}{s}} \\
\ensuremath{\bvslt{\bvor{x}{s}}{{t}}} & \ensuremath{\bvminsf} \\
\ensuremath{\bvslt{\bvand{x}{s}}{{t}}} & \ensuremath{\bvminsf} \\
\ensuremath{\bvslt{\bvneg{x}}{{t}}} & \ensuremath{\bvminsf} \\
\hline
\end{tabular}}


==> table/iv_bvuge.tex <==
{\renewcommand{\arraystretch}{1.1}%
\begin{tabular}{r@{\hspace{1em}}r}
\hline
\textbf{Literal} &  \textbf{Conditional Inverse} \\
\hline
\ensuremath{\bvuge{\bvand{x}{s}}{{t}}} & \ensuremath{s} \\
\ensuremath{\bvuge{\bvneg{x}}{{t}}} & \ensuremath{\bvneg{t}} \\
\ensuremath{\bvuge{\bvudiv{s}{x}}{{t}}} & \ensuremath{0} \\
\ensuremath{\bvuge{\bvor{x}{s}}{{t}}} & \ensuremath{t} \\
\ensuremath{\bvuge{\bvashr{s}{x}}{{t}}} & \ensuremath{\bvand{s}{\bvminsf}} \\
\ensuremath{\bvuge{\bvashr{x}{s}}{{t}}} & \ensuremath{\bvnot{0}} \\
\ensuremath{\bvuge{\bvlshr{x}{s}}{{t}}} & \ensuremath{\bvnot{s}} \\
\ensuremath{\bvuge{\bvlshr{s}{x}}{{t}}} & \ensuremath{0} \\
\ensuremath{\bvuge{\bvshl{x}{s}}{{t}}} & \ensuremath{\bvnot{0}} \\
\ensuremath{\bvuge{\bvadd{x}{s}}{{t}}} & \ensuremath{\bvnot{s}} \\
\ensuremath{\bvuge{\bvurem{x}{s}}{{t}}} & \ensuremath{t} \\
\ensuremath{\bvuge{\bvurem{s}{x}}{{t}}} & \ensuremath{0} \\
\ensuremath{\bvuge{\bvnot{x}}{{t}}} & \ensuremath{0} \\
\hline
\end{tabular}}


==> table/iv_bvugt.tex <==
{\renewcommand{\arraystretch}{1.1}%
\begin{tabular}{r@{\hspace{1em}}r}
\hline
\textbf{Literal} &  \textbf{Conditional Inverse} \\
\hline
\ensuremath{\bvugt{\bvadd{x}{s}}{{t}}} & \ensuremath{\bvnot{s}} \\
\ensuremath{\bvugt{\bvurem{s}{x}}{{t}}} & \ensuremath{0} \\
\ensuremath{\bvugt{\bvurem{x}{s}}{{t}}} & \ensuremath{\bvnot{\bvneg{s}}} \\
\ensuremath{\bvugt{\bvlshr{s}{x}}{{t}}} & \ensuremath{0} \\
\ensuremath{\bvugt{\bvlshr{x}{s}}{{t}}} & \ensuremath{\bvnot{s}} \\
\ensuremath{\bvugt{\bvor{x}{s}}{{t}}} & \ensuremath{\bvnot{s}} \\
\ensuremath{\bvugt{\bvnot{x}}{{t}}} & \ensuremath{0} \\
\ensuremath{\bvugt{\bvand{x}{s}}{{t}}} & \ensuremath{s} \\
\ensuremath{\bvugt{\bvshl{x}{s}}{{t}}} & \ensuremath{\bvnot{0}} \\
\ensuremath{\bvugt{\bvudiv{x}{s}}{{t}}} & \ensuremath{\bvnot{0}} \\
\ensuremath{\bvugt{\bvudiv{s}{x}}{{t}}} & \ensuremath{0} \\
\ensuremath{\bvugt{\bvashr{x}{s}}{{t}}} & \ensuremath{\bvnot{0}} \\
\ensuremath{\bvugt{\bvashr{s}{x}}{{t}}} & \ensuremath{\bvand{s}{\bvminsf}} \\
\ensuremath{\bvugt{\bvneg{x}}{{t}}} & \ensuremath{\bvnot{t}} \\
\hline
\end{tabular}}


==> table/iv_bvule.tex <==
{\renewcommand{\arraystretch}{1.1}%
\begin{tabular}{r@{\hspace{1em}}r}
\hline
\textbf{Literal} &  \textbf{Conditional Inverse} \\
\hline
\ensuremath{\bvule{\bvadd{x}{s}}{{t}}} & \ensuremath{\bvneg{s}} \\
\ensuremath{\bvule{\bvashr{x}{s}}{{t}}} & \ensuremath{0} \\
\ensuremath{\bvule{\bvashr{s}{x}}{{t}}} & \ensuremath{\bvnot{(\bvor{s}{\bvmaxsf})}} \\
\ensuremath{\bvule{\bvor{x}{s}}{{t}}} & \ensuremath{s} \\
\ensuremath{\bvule{\bvand{x}{s}}{{t}}} & \ensuremath{t} \\
\ensuremath{\bvule{\bvlshr{s}{x}}{{t}}} & \ensuremath{s} \\
\ensuremath{\bvule{\bvlshr{x}{s}}{{t}}} & \ensuremath{s} \\
\ensuremath{\bvule{\bvudiv{x}{s}}{{t}}} & \ensuremath{t} \\
\ensuremath{\bvule{\bvudiv{s}{x}}{{t}}} & \ensuremath{\bvnot{0}} \\
\ensuremath{\bvule{\bvmul{x}{s}}{{t}}} & \ensuremath{0} \\
\ensuremath{\bvule{\bvnot{x}}{{t}}} & \ensuremath{\bvnot{t}} \\
\ensuremath{\bvule{\bvshl{x}{s}}{{t}}} & \ensuremath{0} \\
\ensuremath{\bvule{\bvshl{s}{x}}{{t}}} & \ensuremath{\bvminsf} \\
\ensuremath{\bvule{\bvurem{s}{x}}{{t}}} & \ensuremath{s} \\
\ensuremath{\bvule{\bvurem{x}{s}}{{t}}} & \ensuremath{s} \\
\ensuremath{\bvule{\bvneg{x}}{{t}}} & \ensuremath{0} \\
\hline
\end{tabular}}


==> table/iv_bvult.tex <==
{\renewcommand{\arraystretch}{1.1}%
\begin{tabular}{r@{\hspace{1em}}r}
\hline
\textbf{Literal} &  \textbf{Conditional Inverse} \\
\hline
\ensuremath{\bvult{\bvurem{x}{s}}{{t}}} & \ensuremath{s} \\
\ensuremath{\bvult{\bvurem{s}{x}}{{t}}} & \ensuremath{s} \\
\ensuremath{\bvult{\bvand{x}{s}}{{t}}} & \ensuremath{0} \\
\ensuremath{\bvult{\bvadd{x}{s}}{{t}}} & \ensuremath{\bvneg{s}} \\
\ensuremath{\bvult{\bvshl{s}{x}}{{t}}} & \ensuremath{\bvminsf} \\
\ensuremath{\bvult{\bvshl{x}{s}}{{t}}} & \ensuremath{0} \\
\ensuremath{\bvult{\bvor{x}{s}}{{t}}} & \ensuremath{s} \\
\ensuremath{\bvult{\bvnot{x}}{{t}}} & \ensuremath{\bvneg{t}} \\
\ensuremath{\bvult{\bvmul{x}{s}}{{t}}} & \ensuremath{0} \\
\ensuremath{\bvult{\bvneg{x}}{{t}}} & \ensuremath{0} \\
\ensuremath{\bvult{\bvashr{s}{x}}{{t}}} & \ensuremath{\bvnot{(\bvor{s}{\bvmaxsf})}} \\
\ensuremath{\bvult{\bvashr{x}{s}}{{t}}} & \ensuremath{0} \\
\ensuremath{\bvult{\bvlshr{x}{s}}{{t}}} & \ensuremath{s} \\
\ensuremath{\bvult{\bvlshr{s}{x}}{{t}}} & \ensuremath{s} \\
\ensuremath{\bvult{\bvudiv{s}{x}}{{t}}} & \ensuremath{\bvnot{0}} \\
\ensuremath{\bvult{\bvudiv{x}{s}}{{t}}} & \ensuremath{0} \\
\hline
\end{tabular}}


==> table/iv_ne.tex <==
{\renewcommand{\arraystretch}{1.1}%
\begin{tabular}{r@{\hspace{1em}}r}
\hline
\textbf{Literal} &  \textbf{Conditional Inverse} \\
\hline
\ensuremath{\tneqf{\bvnot{x}}{{t}}} & \ensuremath{t} \\
\ensuremath{\tneqf{\bvurem{s}{x}}{{t}}} & \ensuremath{t} \\
\ensuremath{\tneqf{\bvor{x}{s}}{{t}}} & \ensuremath{\bvnot{t}} \\
\ensuremath{\tneqf{\bvmul{x}{s}}{{t}}} & \ensuremath{\bvshl{\bvmaxsf}{t}} \\
\ensuremath{\tneqf{\bvadd{x}{s}}{{t}}} & \ensuremath{\bvnot{(\bvadd{s}{t})}} \\
\ensuremath{\tneqf{\bvlshr{s}{x}}{{t}}} & \ensuremath{\bvneg{t}} \\
\ensuremath{\tneqf{\bvlshr{x}{s}}{{t}}} & \ensuremath{\bvshl{\bvminsf}{t}} \\
\ensuremath{\tneqf{\bvudiv{s}{x}}{{t}}} & \ensuremath{\bvand{t}{\bvminsf}} \\
\ensuremath{\tneqf{\bvudiv{x}{s}}{{t}}} & \ensuremath{\bvlshr{s}{t}} \\
\ensuremath{\tneqf{\bvneg{x}}{{t}}} & \ensuremath{\bvnot{t}} \\
\ensuremath{\tneqf{\bvurem{x}{s}}{{t}}} & \ensuremath{\bvneg{\bvnot{t}}} \\
\ensuremath{\tneqf{\bvand{x}{s}}{{t}}} & \ensuremath{\bvnot{t}} \\
\ensuremath{\tneqf{\bvshl{x}{s}}{{t}}} & \ensuremath{\bvshl{\bvmaxsf}{t}} \\
\ensuremath{\tneqf{\bvshl{s}{x}}{{t}}} & \ensuremath{t} \\
\ensuremath{\tneqf{\bvashr{x}{s}}{{t}}} & \ensuremath{\bvnot{t}} \\
\ensuremath{\tneqf{\bvashr{s}{x}}{{t}}} & \ensuremath{\bvlshr{t}{\bvsub{s}{t}}} \\
\hline
\end{tabular}}

